The Baum-Connes conjecture and proper group actions on affine buildings

We study the possibility of applying a finite-dimensionality argument in order to address parts of the Baum-Connes conjecture for finitely generated linear groups. This gives an alternative approach to the results of Guentner, Higson, and Weinberger concerning the Baum-Connes conjecture for linear groups. For any finitely generated linear group over a field of characteristic zero we construct a proper action on a finite-asymptotic-dimensional CAT(0)-space, provided that for such a group its unipotent subgroups have `bounded composition rank'. The CAT(0)-space in our construction is a finite product of symmetric spaces and affine Bruhat-Tits buildings. For the case of finitely generated subgroup of SL(2,C) the result is sharpened to show that the Baum-Connes assembly map is an isomorphism.

==> conclusion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Conclusion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this thesis we have studied the finite-dimensionality arguments which concern different aspects of the Baum-Connes conjecture with coefficients for linear groups over the fields of characteristic $0$. In this chapter we comment on the limitations of the method developed in this thesis and possible directions of further investigations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proper vs. metrically proper}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this work we have shown that under some assumptions on the unipotent subgroups any finitely generated linear group over a field of characteristic zero admits a proper action on a finite-asymptotic-dimensional space. We are tempted to feed this result into Theorem~\ref{theoremYu}, but for that we need to make sure that the action in question is actually metrically proper.

In general, our construction produces an action on a finite product of symmetric spaces and affine buildings. Notably, while proving properness of the action on a symmetric space we actually proved metrical properness, however that was not the case for the action on the affine buildings part. It could happen that the stabilizer of any vertex in a building is finite or even trivial, while there are infinitely many group elements moving this vertex distance $1$ away.

To illustrate this phenomenon, we recall Example~\ref{exampleBad}. The linear group $G$ in that example is generated by matrices $\m{t}{0}{0}{t^{-1}}$ and $\m{1}{1}{0}{1}$. This group is a subgroup of $SL(2,A)$, where we take the finitely generated ring $A$ to be $\Z[t, t^{-1}]$ so that its field of fractions $\Q(t)$ is just a simple transcendental extension of the rationals. Lemma~\ref{lemmaMainThmValuations} asserts that $A$ is an integral extension of $\Z[t-t^{-1}]$ and produces two discrete valuations on $A$. Since the degree of this extension is $2$, the discrete valuation on $\Z[t-t^{-1}]$ which assigns to any polynomial in $t-t^{-1}$ the opposite of the polynomial's degree has two extensions to $A$. These valuations are
\begin{gather*}
\nu_1(x)=m \quad \mbox{ and } \quad \nu_2(x)=-n,\\
x=z_mt^m+\dots+z_nt^n, \quad z_i\in\Z, \quad  -\infty<m\leqslant n<\infty, \quad z_m\ne0\ne z_n.
\end{gather*}
An element $x$ of $A$ which is integral with respect to both of them has to be a rational integer, so that $\mathcal O=\Z$ in our notation.

A natural action of $G$ on the product of two trees (with respect to valuations $\nu_1$ and $\nu_2$) has isotropy conjugate to subgroups of $SL(2,\Z)$ (Theorem~\ref{theoremMainThmAS}), while an action of $G$ on a hyperbolic plane (in accordance with Theorem~\ref{theoremProperActionSL2Q}) is proper on $SL(2,\Z)$. While the latter action is metrically proper, the former one is not, due to the fact that there are infinitely many elements of $A$ with same valuations $\nu_1$, $\nu_2$ and therefore infinitely many elements of $G$ moving vertices of the trees finite distance away.

We see that the Alperin-Shalen technique of Chapter~\ref{chapterMainTheorem} is not sharp enough to provide a metrically proper action for $G$. However, the technique developed in Chapter~\ref{chapterIntegralCharacteristic} says that the unipotent subgroup $\Gamma$ in the notation of Example~\ref{exampleBad} is not boundedly composed and thus we have a reason to reject $G$ from that perspective.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Fields of positive characteristic}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let $K$ be an infinite field of positive characteristic and let $\Gamma$ be a finitely generated subgroup of $SL(n,K)$. Can we apply the argument presented in this thesis to $\Gamma$ and deduce that $\Gamma$ acts properly on a space of finite asymptotic dimension (provided we imposed the boundedness restriction on the unipotent subgroups of $\Gamma$)?

In our construction we reduce the question to the subgroups of $\Gamma$ of integral characteristic in Chapter~\ref{chapterMainTheorem} via the invocation of Noether Normalization Lemma and construction of finitely many valuations based on the normalized set of generators. This part of the construction applies flawlessly, for the only assumption we took is the infinite number of elements of the ground field $K$.

Then for subgroups of $\Gamma$ of integral characteristic we either embed them into $GL(n,\Q)$ for a suitably chosen $m$ or embed them in different ways into $SL(n,\C)$ and consider the actions on a product of affine buildings and a symmetric space. Either way, subgroups of $\Gamma$ do not have to embed faithfully into a linear group over a field of characteristic $0$ ($\Q$ or $\C$ in our construction), and this part of the argument fails.

It is reasonable to seek for conditions which guarantee that the subgroups of integral characteristic of a given finitely generated matrix group admit a proper action of a finite-asymptotic-dimensional space, and this action extends to the action of $\Gamma$ (for example, finite order of those subgroups, but this is too restrictive).

The case of linear groups over a finite field is trivial, since they are finite and therefore have asymptotic dimension $0$ and satisfy the full Baum-Connes conjecture.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Unipotent subgroups}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In Theorem~\ref{theoremIntCharUnipotentProper} we prove that if all unipotent subgroups of a finitely generated linear group $G$ are uniformly boundedly composed, then there is an action of $G$ on a finite-asymptotic-dimensional space, such that its restriction to any unipotent subgroup of $G$ is proper. Then we deduce that the only obstruction that could prevent a finitely generated linear group from acting properly on a space of finite asymptotic dimension is the possible existence of unipotent subgroups which are not uniformly boundedly composed. Note that it could happen that some group $G$ has unboundedly composed unipotent subgroups (or a sequence of boundedly composed unipotent subgroups with parameter of the composition tending to infinity), but these subgroups do not appear among the isotropy subgroups of the Alperin-Shalen-type action from Chapter~\ref{chapterMainTheorem}. In such a case the action of $G$ that we constructed would still be proper.

Another question concerns the notion of a boundedly composed unipotent subgroup. It is easy to show that any group of this kind has finite asymptotic dimension (Theorem~\ref{theoremIntCharUnipotentProper}). The converse is certainly true for $2\times2$ matrices (Theorem~\ref{theoremIntCharUnipotent2}). While the property of being boundedly composed is an efficient way of checking the finiteness of asymptotic dimension, one can ask whether there exists a sharper condition which is actually equivalent to the uniform boundness of the asymptotic dimension of the unipotent subgroups.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The $\gamma$-element}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

There is a better $K$-theoretic description of the injectivity of the Baum-Connes assembly map, which involves the notion of a $\gamma$-element. The group $\Gamma$ is said to have a \textit{$\gamma$-element} if there exists a $C^*$-algebra $A$ on which it acts properly and elements $D\in KK^{\Gamma}(A,\mathbb C)$ and $\eta\in KK^{\Gamma}(\mathbb C,A)$, called Dirac and dual-Dirac, such that $\gamma=\eta\otimes_AD$ satisfies $p^*\gamma=1$ for the projection $p:\underline{E}\Gamma\rtimes\Gamma\to\Gamma$. If such an element exists, the assembly map is split-injective and is easily described (see~\cite{TuGammaElement}). After the original work~\cite{Kasparov} of Kasparov, introducing the $\gamma$-element  for groups acting properly on a simply connected manifold with non-positive sectional curvature, there have been quite a few attempts to translate his result to analogous geometric situations. Julg and Valette in~\cite{JulgValette} constructed the $\gamma$-element for groups acting properly on a tree, and Kasparov and Skandalis constructed it for groups acting on affine buildings in~\cite{KasparovSkandalis}. There appears a natural question, whether the $\gamma$-element for a group acting on the affine buildings used in Chapter~\ref{chapterMainTheorem} can be ``lifted'' from the isotropy subgroups to the group itself.
